Fast, Provable Algorithms for Isotonic Regression in all $\ell_{p}$-norms

Given a directed acyclic graph $G,$ and a set of values $y$ on the vertices, the Isotonic Regression of $y$ is a vector $x$ that respects the partial order described by $G,$ and minimizes $||x-y||,$ for a specified norm. This paper gives improved algorithms for computing the Isotonic Regression for all weighted $\ell_{p}$-norms with rigorous performance guarantees. Our algorithms are quite practical, and their variants can be implemented to run fast in practice.

==> notation.tex <==
\section{Notation}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "isotonic-nips"
%%% End:


==> runtimeTable.tex <==
\begin{wraptable}{R}{0.65\textwidth}
\caption{Running time in practice}
\label{tab:runtimes}
\begin{center}
\begin{tabular}{|c| c c| c c|}
&
\multicolumn{2}{c|}{\bf 2d Grid} &
\multicolumn{2}{c|}{\bf Random Regular}\\ 
{\#vertices} &
Iterations & 
Time(secs) &
Iterations & 
Time(secs)\\
\hline
$5000$ & $74$ & $11$ &
$78$ &$25$ \\
$10000$ & $78$ & $14$ &
$81$ & $13$ \\
$20000$ & $91$ & $31$ &
$90$ & $51$ \\
$40000$ & $96$ & $60$ &
$91$ & $79$\\
$80000$ & $110$ & $156$ &
$99$ & $141$ 
\end{tabular}
%{\small  We produced a dual certificate to ascertain that the output was correct up to 6 decimal places.}
\end{center}
%\vspace{-15pt}
\end{wraptable}
